Near-Optimal Statistical Query Lower Bounds for Agnostically Learning Intersections of Halfspaces with Gaussian Marginals

We consider the well-studied problem of learning intersections of halfspaces under the Gaussian distribution in the challenging \emph{agnostic learning} model. Recent work of Diakonikolas et al. (2021) shows that any Statistical Query (SQ) algorithm for agnostically learning the class of intersections of $k$ halfspaces over $\mathbb{R}^n$ to constant excess error either must make queries of tolerance at most $n^{-\tilde{\Omega}(\sqrt{\log k})}$ or must make $2^{n^{\Omega(1)}}$ queries. We strengthen this result by improving the tolerance requirement to $n^{-\tilde{\Omega}(\log k)}$. This lower bound is essentially best possible since an SQ algorithm of Klivans et al. (2008) agnostically learns this class to any constant excess error using $n^{O(\log k)}$ queries of tolerance $n^{-O(\log k)}$. We prove two variants of our lower bound, each of which combines ingredients from Diakonikolas et al. (2021) with (an extension of) a different earlier approach for agnostic SQ lower bounds for the Boolean setting due to Dachman-Soled et al. (2014). Our approach also yields lower bounds for agnostically SQ learning the class of "convex subspace juntas" (studied by Vempala, 2010) and the class of sets with bounded Gaussian surface area; all of these lower bounds are nearly optimal since they essentially match known upper bounds from Klivans et al. (2008).

==> intro_extra.tex <==
%--------------------------------------------------------------------------------
\gray{
\clayton{Lead with motivation of intersection of halfspaces via learning halfspaces. Go from there to convex sets, rather than opposite direction}

\manolis{A bigger picture:
Learning Convex sets is a fundamental problem but difficult.
Driven by the convex analysis fact that :
Convex set can be described as the infinite intersection of halfspaces, the lionshare's of approximation has been focused on Intersection of Halfspaces. Give a brief explain what is an oriented-LTF, we present variations of Intersection of Halfspaces speaking about (a),(b),(c)}
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/InOfHalf.png}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}

\manolis{
Throughout, we work with functions that can be represented as intersections of $k$ halfspaces.

\begin{definition}
	We say that $f: \R^n \to \flip$ is an \emph{intersection of $k$ halfspaces} if there exist $w^{(1)}, \dots, w^{(k)} \in \R^n$ and $b^{(1)}, \dots, b^{(k)}$ such that $f(x) = 2\prod_{i=1}^k \indicator{\innerprod{w^{(i)}}{x} \geq b^{(i)}} - 1.$ 
\end{definition}}

\manolis{This is an excellent chance to speak about DNFs and other classes that are expressable via AND of LTFs.
\\ROCCO:PLEASE ELABORATE MORE\\
Intersections of halfspaces: well-studied and important concept class. Mention ``credit assignment'' challenge. 
}
\clayton{Connection to credit assignment... this problem would be easy if we knew which halfspace was responsible for classification outcome; this is what makes it harder than learning one halfspace}

\subsection{Background: Prior algorithms and lower bounds for learning intersections of halfspaces}
 Because of apparent difficulty of learning even an intersection of two halfspaces, much work on this problem has focused on learning under ``nice''\footnote{\manolis{Barlett and Williams define the reasonable distributions}} data distributions such as the uniform distribution on $\bn$ or the Gaussian distribution. Mention \cite{bk97,vempala97,kos04,ks04,vempala10}, note in particular the runtime of \cite{vempala10} as state of the art for learning an intersection of $k$ halfspaces (Maybe brief mention of the approach - PCA then an algorithm on relevant dimensions; the point of mentioning this here would be to convey some intuition towards why such a runtime isn't known for the agnostic  setting, when we explain agnostic stuff later). If we touch on lower bounds here, mention \cite{ks06} (crypto hardness), \cite{ks07} (statistical query for a fixed but somewhat artificial distribution) \cite{ks11} (proper learning hardness - check).

There has also been significant interest in the even harder problem of \emph{agnostically} learning intersections of halfspaces. Agnostic learning of even a single halfspace is a challenging problem (indeed even agnostically learning a disjunction under arbitrary distributions is as hard as learning DNF) so positive results have been for restricted distributions. Mention \cite{kkms} for a single halfspace (and get across that this is the prevailing technique for these agnostic results), describe \cite{kos08} as state-of-the-art for intersections of $k$ halfspaces under Gaussian.  Since these results have resisted improvement, attention has turned to trying to prove lower bounds, and such lower bounds are the subject of this paper.

\subsubsection{Statistical Query learning}
The SQ model provides an attractive setting for lower bounds. (Briefly discuss SQ model, oracle, etc. The above algorithms (realizable and agnostic) are SQ, as are many/most algorithms, so it's interesting to prove lower bounds on agnostic SQ learning. \cite{dftww14} were the first to develop techniques for agnostic SQ lower bounds under ``nice'' distributions (in their case, uniform on $\bn$); briefly sketch their results/techniques (duality, resilience, $L^1$ polynomial approximation bounds). Since then a number of researchers (list papers: [GGK20, DKZ20]) have used various other techniques to give SQ lower bounds for classes related to halfspaces including ReLUs and intersections of halfspaces. (Brief overview of some of that work / techniques, leading up to \cite{dkpz21}). State \cite{dkpz21} results, note their mention (p. 14 just before Theorem 3.5) that  ``it is a plausible conjecture that the right answer is $\Theta(\sqrt{\log k}/\eps^2)$.''\footnote{Explain how they are talking here about the $L^1$ polynomial $\eps$-degree of an intersection of $k$ halfspaces w.r.t. the Gaussian distribution, and give pointer to the result by which this $L^1$ polynomial $\eps$-degree bound would imply $n^{O(\sqrt{\log k}/\eps^)}$ time learning.}

\subsection{Our results: Near-optimal lower bounds for agnostic SQ learning of intersections of halfspaces}

State our results in detail (including convex subspace junta agnostic SQ lower bounds). (Should we have a table?)

\clayton{Table: one row per paper? one for DKPZ, KOS, us. Maybe it would be better as a line to show how much better we are than DKPZ}

\subsection{Relation to previous work}
Explain how for constant $\eps$, these lower bounds almost match the \cite{kos08} algorithmic results (upper bounds) and thus essentially settle the SQ complexity of agnostic learning intersections of halfspaces. (See Clayton's bullets below). Describe the \cite{kos08} MQ lower bounds and explain the difference; highlight the fact that a $k^{\Omega(1)}$ query lower bound for intersection of $k$ halfspaces is not very interesting (and is basically trivial if $k \leq \poly(n)$. Our results in contrast are superpoly$(n)$ for any $k = \omega(1).$


\subsection{Techniques}

We  give two proofs. Explain the ingredients we need from \cite{dkpz21}. Explain how, given those ingredients, the approach hews closer to the original \cite{dftww14} approach.

Overview of first proof.

Overview of second proof.

\subsection{Outline}
(Brief explanation of the structure of the rest of the paper)  



\bigskip \bigskip \bigskip

\clayton{This gray is ``reorganization gray''}
\gray{
We prove the near-optimality of the algorithm presented by \cite{kos08} for agnostically learning functions $f: \R^n \to \flip$ that can be expressed as intersections of $k$ halfspaces with samples drawn iid from the standard multivariate Gaussian distribution $\mnormal$.
They do so by defining a notion of \emph{Gaussian surface area} as follows.\rocco{Maybe this discussion of GSA can go in the techniques section?}

\begin{definition}
	The \emph{Gaussian surface area} of a Boolean-valued function $f: \R^n \to \flip$, for which $\set{x \in \R^n: f(x) = 1}$ is a Borel set, is 
	\[\Gamma(f) = \liminf_{\delta \to 0} \frac{\pr[x \sim \mnormal]{f(x) = -1, \ \exists y \text{ s.t. } \norm[2]{x - y} \leq \delta, f(y) = 1}}{\delta}. \]
	\cite{kos08} defines this quantity in terms of a subset $A \subset \R^n$ rather than a Boolean function, but the two are equivalent.
\end{definition}
}
\manolis{I want to put a plot for the GSA...The color should be a colormap and two convex sets whose limit will explain GSA}
\begin{figure}
\centering
\begin{tikzpicture}[bullet/.style={circle,fill,inner sep=1pt,node contents={}},scale=1]
\shadedraw[red, inner color=red,opacity=0.8]   (0,0)  to[out=105,in=0] ++ 
        (-0.5,0.75) to[out=180,in=105] ++ 
        (-1.,-1.5) to[out=-75,in=180] ++ 
        (1,-0.75) to[out=0,in=-75] cycle;
%\shadedraw[blue,opacity=0.8]  (0.7,1)--(0.7,-1.75)--(1.5,-1.75)--(1.5,1)--cycle;
\draw[red,thick]   (1,-0.75) node[bullet,label=below:$x_1$];
%\draw[blue,thick]   (1,0.5) node[bullet,label=below:$x_2$];
%\draw[blue, thick]  (0.7,1)--(0.7,-1.75);
%\draw[blue]   (1,1.5) node{$\langle a, x \rangle \ge b$};
\draw[thick]   (-0.8,-0.3) node{$F(x)$};
\end{tikzpicture}
\end{figure}

\gray{

They prove the following results:\rocco{I'm not sure to what extent we want to ``foreground'' these results from \cite{kos08} in the introduction - maybe we explain them in the ``Our Results'' section, seems like a natural place to state them (in the context of explaining why our results are optimal)}


\begin{itemize}
	\item Their Theorem~25 shows that any set $\mathcal{C}$ of all Boolean-valued functions $f$ with Gaussian surface area at most $s$ that is closed with respect to affine transformations is agnostically learnable to accuracy $\eps$ in time $n^{O(s^2 / \eps^4)}$.
	\item By Theorem~20, if $f$ is an intersection of at most $k$ halfspaces, then $\Gamma(f) = O(\sqrt{\log k})$. 
	Thus, any intersection of at most $k$ halfspaces is agnostically learnable in time $n^{O(\log(k) / \eps^4)}$. \rocco{This may be improvable to $\eps^2$. Will look into it.}
	\item They provide an information-theoretic lower bound for learning intersections of $k$ halfspaces specifically and functions with Gaussian surface area bounded by $s$ broadly.
	 According to Theorem~26, any learning algorithm that learns the class of all intersections of $k$ halfspaces to constant accuracy (say $\eps = 0.1$) for $k = n^{\Omega(1)}$ and $k = 2^{\Omega(\sqrt{n})}$ must use $k^{\Omega(1)}$ examples.
	 As a corollary, any learning algorithm that learns the class of all functions with Gaussian surface area at most $s$ for $s = \Omega(\sqrt{\log n})$ and $s = O(n^{1/4})$ reequires $2^{\Omega(s^2)}$ membership queries.
   \daniel{Should this just be directly stated as requiring $2^{\Omega(s^2)}$ membership queries? And then giving a translation to what it would imply for SQ algorithms?}
   \clayton{What is the direct connection from SQ algs to MQ algs?}
%	 These bounds are particularly strong because they permit noiseless membership queries.
\end{itemize}

Our contribution is to prove an SQ lower bound on agnostically learning intersections of halfspaces, which is a different learning regime than the MQ lower bound from \cite{kos08}. 
The setting we consider is an ``easier'' one than the \cite{kos08} one, because a small number of MQs can be used to simulate an SQ, when the data distribution is known; on the other hand, an MQ cannot easily be simulated with SQs.
Given the relative easiness of proving lower bounds in our regime, it is natural that we show that the  number of SQs required to learn an intersection of halfspaces is larger than the number of MQs required by \cite{kos08}.
%\rocco{Phrase this differently, since these are in two different regimes and are incomparable}
%These do \emph{not} strictly dominate the \cite{kos08} lower bounds because those consider the stronger learning setting without noise and with membership queries.

Our bounds strengthen a result by \cite{dkpz21}, whose Theorem 1.4 shows that agnostically learning to accuracy $\eps$ the family of all intersections of $k$ halfspaces requires at least $2^{n^{\Omega(1)}}$ SQs or at least one SQ queries with tolerance $n^{-\tilde{\Omega}(\sqrt{\log k}/ \eps)}$.

We first show that our results strictly dominate theirs in the constant accuracy setting, with $\eps = 0.1$.
Then, we show that our results can be extended to match theirs for all $\eps$ and to strictly dominate theirs when $\eps = \omega(\frac{1}{\sqrt{\log k}})$.
\rocco{Preferable to give two theorems and compare them, later on}

To do so, we offer two different approaches, which additionally draw inspiration from \cite{dftww14} and \cite{ds21}.

}}


==> main.tex <==
\input{colt_main}

